Galaxy Properties and UV Escape Fractions During Epoch of Reionization: Results from the Renaissance Simulations

Cosmic reionization is thought to be primarily fueled by the first generations of galaxies. We examine their stellar and gaseous properties, focusing on the star formation rates and the escape of ionizing photons, as a function of halo mass, redshift, and environment using the full suite of the {\it Renaissance Simulations} with an eye to provide better inputs to global reionization simulations. This suite, carried out with the adaptive mesh refinement code Enzo, is unprecedented in terms of their size and physical ingredients. The simulations probe overdense, average, and underdense regions of the universe of several hundred comoving Mpc$^3$, each yielding a sample of over 3,000 halos in the mass range $10^7 - 10^{9.5}~\Ms$ at their final redshifts of 15, 12.5, and 8, respectively. In the process, we simulate the effects of radiative and supernova feedback from 5,000 to 10,000 metal-free (Population III) stars in each simulation. We find that halos as small as $10^7~\Ms$ are able to form stars due to metal-line cooling from earlier enrichment by massive Population III stars. However, we find such halos do not form stars continuously. Using our large sample, we find that the galaxy-halo occupation fraction drops from unity at virial masses above $10^{8.5}~\Ms$ to $\sim$50\% at $10^8 ~\Ms$ and $\sim$10\% at $10^7~\Ms$, quite independent of redshift and region. Their average ionizing escape fraction is $\sim$5\% in the mass range $10^8 - 10^9~\Ms$ and increases with decreasing halo mass below this range, reaching 40--60\% at $10^7~\Ms$. Interestingly, we find that the escape fraction varies between 10--20\% in halos with virial masses $\sim 3 \times 10^9~\Ms$. Taken together, our results confirm the importance of the smallest galaxies as sources of ionizing radiation contributing to the reionization of the universe.

==> discussion.tex <==
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "draft"
%%% End:

